The Helping Hand: An Assistive Manipulation Framework Using Augmented Reality and a Tongue-Drive Interfaces

A human-in-the-loop system is proposed to enable collaborative manipulation tasks for person with physical disabilities. Studies show that the cognitive burden of subject reduces with increased autonomy of assistive system. Our framework obtains high-level intent from the user to specify manipulation tasks. The system processes sensor input to interpret the user's environment. Augmented reality glasses provide ego-centric visual feedback of the interpretation and summarize robot affordances on a menu. A tongue drive system serves as the input modality for triggering a robotic arm to execute the tasks. Assistance experiments compare the system to Cartesian control and to state-of-the-art approaches. Our system achieves competitive results with faster completion time by simplifying manipulation tasks.

==> figSystem.tex <==
\begin{figure*}[t]
  \vspace*{0.1in}
  \begin{tikzpicture}[inner sep=0pt]
    \node[anchor=south west] (SD) at (0in,0in) 
      {\includegraphics[width=1.25\columnwidth,clip=yes,trim=0in 0.5in 0in 0in]{./../figures/system.png}};
    \node[anchor=north west, xshift=0.15in] at (SD.north east)
      {\includegraphics[width=1in]{./../figures/meta_AR1_devkit.png}};
    \node[anchor= west, xshift=0.45in] (TDSL)at (SD.east)
      {\includegraphics[width=1.5in]{./../figures/TDS_lady.png}};
    \node[anchor=west, xshift=-0.1in, yshift=0.05in] at (TDSL.east)
      {\includegraphics[width=0.75in]{./../figures/TDS_inputs.png}};
  \end{tikzpicture}
  \caption{Diagram of system components: hardware and software.
  \label{system}}
\end{figure*}




==> review.tex <==
%Human computer interface has been developed for several years. It is
%widely used for assistive technology for disabled population. There are
%countless system designs for human-robot interface. In this review, we
%focus on the key components in our system choices, which are the
%tongue-drive and augmented reality glasses. We also review those system
%works which has similar design as a whole. 

%Many human robot interface has been developed with advanced
%technologies. Among those popular interface, sip-and-sup is one of the
%most common used approach due to its low cost and easy to operate.
%However, sip-and-sup only provides limited commands and thus it is
%prevented from being used for more complicated operation or human
%control. Eye-tracker \cite{poole2006eye, chin2008integrated} is another
%common choice since it is more convenient without moving the head or
%large body parts. User can input the command by simply moving the eyes
%and the detector can identify the difference for generating input
%signals. The drawback of this interface is that it will need a detector
%been put in front of the user's face and results in block of view. The
%other choice is the EMG signal \cite{sears1991proportional,
%robinson1995proportional, ahsan2009emg, farina2014extraction}. EMG is
%used to detect the signal on the human skin and translates the signal
%into higher level intent. However, EMG is commonly be affected by noise
%and results in generating inconsistency with human intent. Furthermore,
%with the advance of speech recognition \cite{el2011survey,
%harada2006vocal, shneiderman2000limits, bourlard2012connectionist,
%zeng2009survey }, human even healthy population rely on voice to
%communicate with computer or smart phone. It is efficient but it may be
%inconvenient in certain area such as library or in public. Also it may
%easily be affected by noise with surroundings. Tongue-drive system, as
%our choice, use human tongue to be the controller for sending commands.
%Human tongue is flexible in the way that it is possible to reach several
%point in human mouth. If we translate the pose into signal by applying
%magnetic field, it is of value and can be used to generate complicated
%command such as controlling wheelchair, robotics arm or even texting on
%the phone.     

Assistive robots for persons with disabilities increase user
independence and enhance physical functionality. They can be broadly
categorized into companion robots apart from wheelchairs, and robotic
devices integrated with wheel chairs, for which the wheelchair mounted
robotic arm (WMRA) is one such example \cite{KiWaBe_ToM[2012]}. 
The former category consists of static manipulators and mobile
manipulators. Static manipulators are typically installed or placed
where needed and cannot move on their own.  Mobile manipulators can aid
a person with different tasks that share common manipulation strategies 
\cite{ChEtAl_RAM[2013],DeEtAl_AR[2008],GrHaSc_AR[2004],LaEtAl_APMR[2009]}. 
The work described here fits in the static manipulator category.

Early assistive manipulation research focused on using existing
interfaces (joystick, touch-screen) to directly control the robot arms,
much like most commercial products today. Contemporary work focuses on
supervisory or shared control with efforts going towards designing
interfaces for facilitating and simplifying the user experience
improving the design for performance and and improving perception,
planning, and control algorithms for increased autonomy
\cite{DuLeMa_ICORR[2007],EdKe_ROMAN[2007],GrKe_RSSW[2016],
KiEtAl_TSMCA[2012],KieEtAl_ToM[2014],ChWaCo_JSCM[2013]}.  work in This
paper describes how to leverage contemporary advances in computer vision
and robotic planning to increase the autonomy of assistive manipulation
robots, while using new tongue-drive technology for hands-free operation.

A key component of the assistive robotic system is the use of augmented
reality (AR) glasses as the interface for communicating high-level human
intents. Augmented reality glassed, first designed for gaming,
allow users to visualize virtual objects in real environments.
With augmented reality glasses a user can control a virtual menu or
program \cite{azuma1997survey}.  Recently AR has been applied to
the rehabilitation and assistive systems fields.  Explored use cases
include education for cognitive disable elementary school children
\cite{richard2007augmented}, 
and for surgical robotics \cite{wen2014hand} which described a framework
for human robot collaboration, whereby hand gestures are used for
communication with the robot.  Additionally, \cite{markovic2014stereovision} 
develops a human-robot collaborative mechanism involving a 
hand prostheses to assess the grasping ability of the user to
provide grasping feedback via AR. 

%Compare to
%\cite{markovic2014stereovision}, we provide a more autonomous system
%framework that our robot arm identifies best grasp and perform path
%planning for reaching the target. 
A recently developed system whose overall design is similar 
to the one described here \cite{wang2017robotic} uses eye gaze and EEG
as the two input modalities.  The user can perform pick and place
activities with a low DOF robotic arm by fixating their gaze and
activating the EEG via thought.  Intermediate phases of the routine must
be controlled by the user through the assistance of a nearby monitor
that provides augmented reality (AR) feedback.  The AR approach was shown to
improve task performance (time and error) relative to the lack of AR.

Compared to previous approaches, our input modalities are a head-mounted AR and a tongue drive system (TDS). A headworn AR system through head fixation prevents gaze to be broken from objects of interest, provides flexibility without extra monitor, and improves autonomy interacting with environment (such as to directly select placing positions with overlapping scenes). The TDS, on the other hand, serves as a versatile interface to communicate to AR with minimum burden under quite or noisy environment. Besides, our work seeks to develop a more autonomous robotic system through the integration of modern computer vision algorithms and advanced robotic planning methods. The overall proposed system communicates high level intent to robotic arm, and simplifies complicated manipulation processes for human desired tasks.   



%proposed a human-in-the-loop system
%with AR which focuses on using EEG with eye gaze position as the
%feedback to control simple robotic arm movement. 

%Whereas in our scenario
%we consider more realistic situation to grasp object on office tale like
%plane with 7DOF arm for more complicated pose with constraints. We apply
%TDS so an extra monitor is not requirement and thus our system is more
%flexible. 

%\cite{wang2017robotic} also proposed an AR-based collaborative
%system for grasping. Whereas directly display on AR glasses, they
%project the AR of object (point cloud like) to augment with target
%object and show it on monitor. By moving the eyebrow the user is able to
%select the desired grasp and require the robotics arm to perform
%manipulation task. Our work aim at providing autonomy of system and
%maintaining the flexiblity of users. By combining tongue-drive system
%with augmented reality glasses, we are able to communicate high level
%intent with the assistive robotic arm to accomplish human desired
%manipulation tasks.      
%
%Also, a TDS interface in our system
%works as a more general framework for even people with upper limbs
%disabled. 

